Stochastic Chebyshev Gradient Descent for Spectral Optimization

A large class of machine learning techniques requires the solution of optimization problems involving spectral functions of parametric matrices, e.g. log-determinant and nuclear norm. Unfortunately, computing the gradient of a spectral function is generally of cubic complexity, as such gradient descent methods are rather expensive for optimizing objectives involving the spectral function. Thus, one naturally turns to stochastic gradient methods in hope that they will provide a way to reduce or altogether avoid the computation of full gradients. However, here a new challenge appears: there is no straightforward way to compute unbiased stochastic gradients for spectral functions. In this paper, we develop unbiased stochastic gradients for spectral-sums, an important subclass of spectral functions. Our unbiased stochastic gradients are based on combining randomized trace estimators with stochastic truncation of the Chebyshev expansions. A careful design of the truncation distribution allows us to offer distributions that are variance-optimal, which is crucial for fast and stable convergence of stochastic gradient methods. We further leverage our proposed stochastic gradients to devise stochastic methods for objective functions involving spectral-sums, and rigorously analyze their convergence rate. The utility of our methods is demonstrated in numerical experiments.

==> proof_thm1.tex <==
\subsection{Proof of Lemma \ref{lem:unbiased}}
An analytic function $f$ has an (unique) infinite Chebyshev series expansion:
$$
f(x) = \sum_{j=0}^\infty b_j T_j(x).
$$
and we remind that 
$$
\wpn{x} = \sum_{j=0}^n \frac{b_j}{1 - \sum_{i=0}^{j-1} q_i} T_j(x).
$$
\iffalse
By the definition of $\wpn{x}$, we can easily show that it is an unbiased estimator of $f(x)$:
\begin{align*}
\mathrm{E}_n\left[ \wpn{x}\right] &= \sum_{n=0}^\infty q_n \wpn{x}= \sum_{n=0}^\infty q_n\sum_{j=0}^n \frac{b_j}{1 - \sum_{i=0}^{j-1} q_i} T_j(x)\\
&= \sum_{j=0}^\infty \left(\sum_{n=j}^\infty q_n\right) \frac{b_j}{1 - \sum_{i=0}^{j-1} q_i} T_j(x)\\
&= \sum_{j=0}^\infty b_j T_j(x) = f(x).
\end{align*}
where $\mathrm{E}_n[\cdot]$ is the expectation over random degree $n$ 
from distribution $\{q_n\}$
and the last inequality holds from that $\sum_{i=0}^\infty q_i = 1$.
\fi
{To prove that $\mathrm{E}_n\left[ \wpn{x}\right] = f(x)$, we define two sequences:
\begin{align*}
&A_{M} \coloneqq \sum_{j=0}^{M} \sum_{n=j}^{M} q_n \frac{b_j T_j(x)}{1 - \sum_{i=0}^{j-1} q_i}, \\
&B_{M,K} \coloneqq \sum_{j=0}^{M} \sum_{n=j}^{K} q_n \frac{b_j T_j(x)}{1 - \sum_{i=0}^{j-1} q_i}.
\end{align*}
Then, it is easy to show that
\begin{align*}
\lim_{M \to \infty} A_M 
&= \sum_{j=0}^\infty \sum_{n=j}^\infty q_n\frac{b_j T_j(x)}{1 - \sum_{i=0}^{j-1} q_i} \\
&= \sum_{n=0}^\infty q_n \left(\sum_{j=0}^n \frac{b_j T_j(x)}{1 - \sum_{i=0}^{j-1} q_i} \right) \\
&= \sum_{n=0}^\infty q_n \wpn{x} = \mathrm{E}_n\left[ \wpn{x}\right],
% = \sum_{i=0}^\infty q_i \left(\sum_{j=0}^n \frac{b_j T_j(x)}{1 - \sum_{k=0}^{j-1} q_k} \right)
% = \mathrm{E}_n \left[ \wpn{x}\right]
\end{align*}
and
\begin{align*}
\lim_{M,K \to \infty} B_{M,K} 
&= \lim_{M \to \infty} \sum_{j=0}^{M} \left( \sum_{n=j}^{\infty} q_n\right) \frac{b_j T_j(x)}{1 - \sum_{i=0}^{j-1} q_i} \\
&= \lim_{M \to \infty} \sum_{j=0}^{M} b_j T_j(x) = f(x).
\end{align*}
However, in general, $A_M$ and $B_{M,K}$ do not converge to the same values, i.e.,
$$
\lim_{M \to \infty} A_M \neq \lim_{M,K \to \infty} B_{M,K}.
$$
Now assume that sufficiently large $M \geq K$. From the condition that $\lim_{n \to \infty} \sum_{i=n+1}^\infty q_i \wpn{x}$ 
we have
\begin{align*}
&\mathrm{E}_n\left[ \wpn{x}\right] - f(x) = \lim_{M,K \to \infty}  \left( A_M - B_{M,K} \right) \\
&= \lim_{M,K \to \infty}  \left(\sum_{j=0}^M \sum_{n=M+1}^K q_n \frac{b_j T_j(x)}{1 - \sum_{i=0}^{j-1} q_i}\right) \\
&= \lim_{M,K \to \infty}  \left( \sum_{n=M+1}^K q_n \right) \left( \sum_{j=0}^M \frac{b_j T_j(x)}{1 - \sum_{i=0}^{j-1} q_i} \right)\\
&= \lim_{M \to \infty}  \left( \sum_{n=M+1}^\infty q_n \right) \left( \sum_{j=0}^M \frac{b_j T_j(x)}{1 - \sum_{i=0}^{j-1} q_i} \right) \\
&= \lim_{M \to \infty} \left( \sum_{n=M+1}^\infty q_n \right) \widehat{p}_M(x) = 0.
%&= \left( \lim_{M,K \to \infty} \sum_{k=M+1}^K q_k \right) \left(\lim_{M \to \infty} \sum_{j=0}^M \frac{b_j T_j(x)}{1 - \sum_{i=0}^{j-1} q_i} \right)\\
%&= \left( \lim_{M,K \to \infty} \sum_{k=M+1}^K q_k \right)
\end{align*}
Therefore, we can conclude that $\wpn{x}$ is an unbiased estimator of $f(x)$.}
In addition, this also holds for matrix bilinear form due to its linearity:
\begin{align*}
%&\mathrm{E}_n\left[ \wpn{A} \right] = f(A) \\
\mathrm{E}_n\left[ \vv^\top \wpn{A} \vv \right] = \vv^\top f(A) \vv.
\end{align*}
By taking expectation over Rademacher random vector $\vv$,
we establish the unbiased estimator of spectral sums:
\begin{align*}
\mathrm{E}_{\vv} \mathrm{E}_n\left[ \vv^\top \wpn{A} \vv \right]
=\mathrm{E}_{\vv}\left[ \vv^\top f(A) \vv\right]
=\tr{f(A)},
\end{align*}
%where $\mathrm{E}_\vv[\cdot]$ is the expectation over Rademacher random vectors.
%Since we choose random vector $\vv$ and degree distr
%Since polynomial $\wpn{A}$ is differentiable with respect to $A$,
%it is possible to exchange derivative operator and expectation
For fixed $\mathbf{v}$ and ${n}$, the function 
$h(\theta) \coloneqq \vv^\top \hat{p}_n(A(\theta)) \vv$ is a linear
combination of all entries of $A$, so the fact that all 
partial derivatives $\partial A_{j,k} /\partial \theta_i$
exist and are continuous implies that the partial derivatives of $h$
with respect to $\theta_1,\dots,\theta_{d^\prime}$ exist and are continuous.
Thus, by the Leibniz rule, the gradient operator and expectation operator can be interchanged:
\begin{align*}
\nabla_\theta \tr{f(A)} 
&= \nabla_\theta \E{\vv^\top \wpn{A} \vv} 
= \E{\nabla_\theta \vv^\top \wpn{A} \vv}.
%\nabla_A \mathrm{E}\left[ \vv^\top \wpn{A} \vv \right]
%= \mathrm{E}\left[ \nabla_A \vv^\top \wpn{A} \vv \right]
\end{align*}
This completes the proof of Lemma \ref{lem:unbiased}.

\subsection{Proof of Lemma \ref{lmm:2}}
The squared error can be written as
\begin{align*}
&\norm{\widehat{p}_n - f}_C^2 
= \norm{\widehat{p}_n - p_n + p_n - f}_C^2 \\
&= \norm{p_n - f}_C^2 + 2 \inner{p_n - f , \widehat{p}_n - p_n}_C + \norm{\widehat{p}_n - p_n}_C^2 \\
&\overset{(\dagger)}{=} \norm{p_n - f}_C^2 + \norm{\widehat{p}_n - p_n}_C^2 \\
&= \norm{\sum_{j=n+1}^\infty b_j T_j(x)}_C^2 + \norm{\sum_{j=1}^n \frac{\sum_{k=0}^{n-1}q_n}{1 - \sum_{k=0}^{n-1}q_n} b_j T_j(x)}_C^2 \\
&\overset{(\ddagger)}{=} 
\frac{\pi}{2} \sum_{j=n+1}^\infty b_j^2 + 
\frac{\pi}{2} \sum_{j=1}^n \left( \frac{\sum_{k=0}^{n-1}q_n}{1 - \sum_{k=0}^{n-1}q_n} b_j \right)^2.
\end{align*}
Both the third equality $(\dagger)$ and the last equality $(\ddagger)$ 
come from the orthogonality of Chebyshev polynomials and the following facts:\
\begin{align*}
p_n - f \ &: \text{linear combination of } \ T_{n+1}(x), T_{n+2}(x), \cdots, \\
\widehat{p}_n - p_n \ &: \text{linear combination of } \ T_0(x), \cdots , T_n(x).
\end{align*}
The objective variance can be computed as follow:
\begin{align*}
& \frac{2}{\pi} \E{\norm{\widehat{p}_n - f}_C^2 } = \frac{2}{\pi} \sum_{n=0}^\infty q_n \norm{\widehat{p}_n - f}_C^2 \\
&= q_0 \sum_{j=1}^\infty b_j^2 
+ \sum_{n=1}^\infty q_n \left(  \sum_{j=1}^n \left(\frac{b_j\sum_{k=0}^{j-1} q_k}{1 - \sum_{k=0}^{j-1} q_k} \right)^2 + \sum_{j=n+1}^\infty b_j^2 \right) \\
&= \sum_{j=1}^\infty b_j^2 \left( q_0 + \sum_{n=1}^{j-1} q_n + \left( \frac{\sum_{k=0}^{j-1} q_k}{1 - \sum_{k=0}^{j-1} q_k}\right)^2 \sum_{n=j}^\infty q_n \right) \\
&= \sum_{j=1}^\infty b_j^2 \left( \sum_{n=0}^{j-1} q_n + \left( \frac{\sum_{n=0}^{j-1} q_n}{1 - \sum_{n=0}^{j-1} q_n}\right)^2 \left( 1 - \sum_{n=0}^{j-1} q_n \right) \right) \\
&= \sum_{j=1}^\infty b_j^2 \left( \sum_{n=0}^{j-1} q_n +  \frac{\left(\sum_{n=0}^{j-1} q_n\right)^2}{1 - \sum_{n=0}^{j-1} q_n} \right) \\
&= \sum_{j=1}^\infty b_j^2 \left( \frac{\sum_{n=0}^{j-1} q_n}{1 - \sum_{n=0}^{j-1} q_n} \right) 
%&= \sum_{j=1}^\infty b_j^2 \left( \frac{1}{1 - \sum_{n=0}^{j-1} q_n} \right) - \sum_{j=1}^\infty b_j^2.
\end{align*}
This completes the proof of Lemma \ref{lmm:2}

\subsection{Proof of Theorem \ref{thm:optdist}}
The problem \eqref{eq:degprob} is equivalent to minimize that
\begin{align*}
\sum_{j=1}^{\infty} \rho^{-2j} \left( \frac{1}{1 - \sum_{n=0}^{j-1}q_n} \right)
\end{align*}
and the equality conditions can be written as%are equivalent with the following:
\begin{align*}
N = \sum_{n=1}^\infty n q_n 
%= \sum_{n=1}^\infty \left( \sum_{j=1}^n 1 \right)q_j 
= \sum_{j=1}^\infty \sum_{n=j}^\infty q_n
= \sum_{j=1}^\infty \left( 1 - \sum_{n=0}^{j-1} q_n \right).
\end{align*}
For simplicity, we change the variables as for $j\geq 1$
\begin{align} \label{eq:changevars}
x_0 := \frac{1}{1-q_0}, \ \ 
x_j := \frac{1}{1 - \sum_{n=0}^{j} q_n}
- \frac{1}{1 - \sum_{n=0}^{j-1} q_n}
%\quad \text{for} \ \ j\geq 1,
\end{align}
which implies that $x_0 \geq 1$ and $x_n \geq 0$ for $n \geq 1$.
The objective function becomes 
\begin{align*}
\sum_{j=1}^\infty \frac{1}{\rho^{2j}} \left( \sum_{n=0}^{j-1} x_n \right)
= \sum_{n=0}^\infty x_n \left( \sum_{j=n}^\infty \frac1{\rho^{2j}}\right),
\end{align*}
and the conditions are considered with variable $x_j$:
\begin{align} \label{eq:cond}
\sum_{j=0}^\infty \frac{1}{\sum_{n=0}^j x_n} = N,
%\qquad x_0 \geq 1, \ \ x_n \geq 0 \quad \text{for } \ n \geq 1.
\end{align}
where $x_0 \geq 1, x_n \geq 0$ for $n \geq 1$. Now We define the Lagrangian as
\begin{align*}
%\mathcal{L}\left( \{ x_j: j\geq 0\}, \{ \eta_j: j \geq 0\}, \lambda, \right)
\mathcal{L}( x_j, &\eta_j, \lambda) 
:= \sum_{n=0}^\infty x_n \left( \sum_{j=n}^\infty \frac1{\rho^{2j}}\right) \\
&+ \lambda \left(\sum_{j=0}^\infty \frac{1}{\sum_{n=0}^j x_j} - N\right) 
+ \eta_0 \left( 1- x_0\right) - \sum_{j=1}^\infty \eta_j x_j
\end{align*}
where $\{\eta_j : j \geq 0\}$ and $\lambda$ are the Lagrangian multipliers of 
equality and inequality condition, respectively.
We note that the problem is {\it convex} so that any solution satisfying KKT conditions is optimal. 
The corresponding KKT conditions are following:
\begin{itemize}
\item {\bf Stationary.} For $j \geq 0$,
\begin{align} \label{eq:kkt1}
\frac{\partial \mathcal{L}}{\partial x_j}
&= \left(\sum_{n=j}^\infty \frac1{\rho^{2(n+1)}}\right) \nonumber \\
&- \lambda \left( \sum_{i=j}^\infty \frac1{\left(\sum_{n=0}^i x_n \right)^2}\right) 
- \eta_j = 0,
%\quad \text{for } \ j\geq 0,
\end{align}
\item {\bf Primal feasibility.} For $j \geq 1$, 
\begin{align} \label{eq:kkt2}
\sum_{j=0}^\infty \frac{1}{\sum_{n=0}^j x_n} = N,
\ \ x_0 \geq 1, \ \ x_j \geq 0,
\end{align}
\item {\bf Dual feasibility.} For $j \geq 0$, 
\begin{align} \label{eq:kkt3}
\eta_j \geq 0,
\end{align}
\item {\bf Complementary slackness.} For $j \geq 1$,
\begin{align} \label{eq:kkt4}
\eta_0 \left( 1- x_0\right) = 0, \ \ \eta_j x_j = 0.
\end{align}
\end{itemize}

{\bf Case 1.} $\eta_j = 0$ for all $j \geq 0$.
\\~\\
In this case, it is satisfied with dual feasibility \eqref{eq:kkt3} and complementary slackness \eqref{eq:kkt4}.
Substracting consecutive stationary conditions \eqref{eq:kkt1}, we have for $j\geq 0$
\begin{align*}
\frac{\partial \mathcal{L}}{\partial x_{j}} - \frac{\partial \mathcal{L}}{\partial x_{j+1}}
= \frac{1}{\rho^{2(j+1)}} - \lambda \frac{1}{\left( \sum_{n=0}^j x_n \right)^2}
= 0 %\ \ \text{for } \ j \geq 0.
\end{align*}
Putting them together into the equality condition \eqref{eq:cond} gives
\begin{align*}
N = \sum_{j=0}^\infty \frac{1}{\sum_{n=0}^j x_n} = \sum_{j=0}^\infty \frac{1}{\sqrt{\lambda} \ \rho^{j+1}} = \frac1{\sqrt{\lambda}\left(\rho - 1\right)}.
\end{align*}
and $\sqrt{\lambda} = \frac1{N \left(\rho-1\right)}$.
Therefore, we obtain the solution that
$x_0 = \rho / \left(N \left(\rho-1\right)\right), \ x_j = \rho^{j} / N$
for $j \geq 1$.
%  \ \ \text{for } j \geq 1$
%, we have
%\begin{align*}
%\sum_{j=0}^\infty \frac{1}{\rho^{j+1}\sqrt{\lambda}} = N
%\end{align*}
%and thus $\lambda = 1 / N (\rho-1)$ and
%\begin{align*}
%x_0 = \frac1N \frac{\rho}{\rho-1}, \ \ x_j = \frac1N \rho^j  \ \ \text{for } j \geq 1.
%\end{align*}
However, it is feasible only if $N \leq \frac{\rho}{\rho-1}.$
Plugging $\{x_j : j \geq 0 \}$ back into \eqref{eq:changevars}, we get
\begin{align} \label{eq:sol1}
q_n 
= \begin{cases}
1 - N \left( 1 - \frac{1}{\rho} \right) \quad  &\text{for } \ n = 0, \\
N \left( 1 - \frac1\rho \right)^2 \frac{1}{\rho^{n-1}} \quad &\text{for } \ n\geq 1.
\end{cases}
\end{align}
In summary, if $N$ is small, i.e., $N \leq \frac{\rho}{\rho-1}$, we have the optimal solution \eqref{eq:sol1}.
\\~\\
{\bf Case 2.} $\eta_j = 0$, $j\geq k+1$ and $\eta_j \neq 0$, $j \leq k$ for some $k \geq 0$
\footnote{If $k=-1$, it is exactly same as the case (1).}. 
\\~\\
By the complementary slackness \eqref{eq:kkt4}, 
we have $x_0 = 1$ and $x_j = 0$ for $1\leq j \leq k$. Similarly, we substract the consecutive stationarity and get
\begin{align} \label{eq:case2}
\frac{1}{\sum_{n=0}^j x_n} = \frac{1}{\sqrt{\lambda}} \frac{1}{\rho^{j+1}}
 \quad \text{for } \ j \geq k+1.
\end{align}
Putting them together into \eqref{eq:cond} gives
\begin{align*}
N &= \sum_{j=0}^\infty \frac{1}{\sum_{n=0}^j x_n}
= k+1 + \frac{1}{\sqrt{\lambda}} \sum_{j=k+1}^\infty \frac{1}{\rho^{j+1}}\\
&= k+1 + \frac{1}{\sqrt{\lambda} \ \rho^{k+1} \left( \rho - 1\right)}
\end{align*}
which leads to that $\sqrt{\lambda} = \frac1{\left(N-k-1\right)\rho^{k+1}\left(\rho-1\right)}$.
Therefore, we obtain the solution from \eqref{eq:case2}:
\begin{align} \label{eq:solx}
x_{j} = 
\begin{cases}
1 \quad &\text{for } \ j=0, \\
0 \quad &\text{for } \ 1 \leq j \leq k, \\
\frac{1}{N - k - 1} \frac{\rho}{\rho-1} - 1 \quad &\text{for } \ j=k+1, \\
\frac{1}{N - k - 1} \rho^{j - k - 1} \quad &\text{for } \ j \geq k+2.
\end{cases}
\end{align}
The inequality in primal feasibility \eqref{eq:kkt2} %, i.e., $x_j \geq 0$ for $j\geq k+1$, 
implies that
\begin{align} \label{eq:k1}
\frac{\rho}{\rho-1} \geq N-k-1 \quad \text{and} \quad k \leq N-1.
\end{align}
In addition, we need to check whehter 
the dual feasibility \eqref{eq:kkt3} is satisfied, 
i.e., $\eta_j > 0$ for $j \leq k$.
From the fact that
\begin{align*}
\eta_k &= \frac{1}{\rho^{2k+2}}\left(1 - \frac1{\left(N-k-1\right)^2\left(\rho-1\right)^2}\right), \\
\eta_{j-1} - \eta_j &= \frac{1}{\rho^{2k+2}}\left( \rho^{2(k+1-j)} - 
\frac1{\left(N-k-1\right)^2\rho^{2k+2}\left(\rho-1\right)^2}\right)
%\qquad \text{for} \ j \leq k,
\end{align*}
for $j \leq k$, it is enough that
\begin{align} \label{eq:k2}
N-k-1 > \frac{\rho}{\rho-1}-1.
\end{align}
Since $k$ is an integer and from \eqref{eq:k1} and \eqref{eq:k2},
we choose $k = N-1-\lfloor \frac{\rho}{\rho-1}\rfloor$.
Plugging back all together into \eqref{eq:changevars}, we obtain the optimal as
\begin{align} \label{eq:sol2}
q_n = 
\begin{cases}
0 \quad 
&\text{for } \ n \leq N-1-\left\lfloor \frac{\rho}{\rho - 1} \right\rfloor,\\
1 - \left\lfloor \frac{\rho}{\rho - 1} \right\rfloor \left( 1 - \frac{1}{\rho}\right) 
&\text{for } \ n = N-\left\lfloor \frac{\rho}{\rho - 1} \right\rfloor,\\
\left\lfloor \frac{\rho}{\rho - 1} \right\rfloor \left( 1 - \frac{1}{\rho}\right)^2 \frac{1}{\rho^{n-1}}
&\text{for } \ n = N-\left\lfloor \frac{\rho}{\rho - 1} \right\rfloor.
\end{cases}
\end{align}
In summary, if $N > \frac{\rho}{\rho-1}$, the optimal solution is that of \eqref{eq:sol2}.

One can easily check that both solution \eqref{eq:sol1} and \eqref{eq:sol2} 
satisfy with $\lim_{n\to \infty}\sum_{i=n+1}^\infty q^{*}_i \widehat{p}_n(x) = 0$
from the facts that $\abs{\sum_{i=n+1}^\infty q^{*}_i} = O(\rho^{-n})$ and $\abs{\widehat{p}_n(x)}=O(n)$.

